Deep Networks as Logical Circuits: Generalization and Interpretation

Not only are Deep Neural Networks (DNNs) black box models, but also we frequently conceptualize them as such. We lack good interpretations of the mechanisms linking inputs to outputs. Therefore, we find it difficult to analyze in human-meaningful terms (1) what the network learned and (2) whether the network learned. We present a hierarchical decomposition of the DNN discrete classification map into logical (AND/OR) combinations of intermediate (True/False) classifiers of the input. Those classifiers that can not be further decomposed, called atoms, are (interpretable) linear classifiers. Taken together, we obtain a logical circuit with linear classifier inputs that computes the same label as the DNN. This circuit does not structurally resemble the network architecture, and it may require many fewer parameters, depending on the configuration of weights. In these cases, we obtain simultaneously an interpretation and generalization bound (for the original DNN), connecting two fronts which have historically been investigated separately. Unlike compression techniques, our representation is. We motivate the utility of this perspective by studying DNNs in simple, controlled settings, where we obtain superior generalization bounds despite using only combinatorial information (e.g. no margin information). We demonstrate how to "open the black box" on the MNIST dataset. We show that the learned, internal, logical computations correspond to semantically meaningful (unlabeled) categories that allow DNN descriptions in plain English. We improve the generalization of an already trained network by interpreting, diagnosing, and replacing components the logical circuit that is the DNN.

==> insightslowres.tex <==
\subsection{Finding the Right Question}
Note that one is \textit{not} always guaranteed small generalization error. There are many settings where DNNs under-perform and have high generalization error. For our purposes, it suffices to recall that when the inputs and outputs $(X,Y)\sim\pdata$ are actually independent, e.g., $Y|X\sim Bernoulli(1/2)$, neural networks still obtain zero empirical risk, which implies the generalization error can be arbitrarily bad in the worst case \citep{Zhang2017}. 
% Some contemplation on this counterexample brings the realizati,on that in order to conclude with confidence that
From this, we can conclude that making either an explicit or implicit assumption about the dataset, the data, or both, is \textit{strictly necessary} and unavoidable. At the very least, one must make an assumption which rules out random labels with high probability. 
% However, we will frame our discussion in terms of properties of the dataset instead of the more abstract data distribution, though both approaches have merit\footnote{One can exchange a dataset property, "$\trainS$ has property P", for a data distribution property: "$m$ samples from $\pdata$ have property P with high probability". So, whether the dataset or data distribution plays a more central role in the discussion is probably just a matter of taste.}.

Notice that the only procedural distinction between a DNN that will generalize and one that will memorize is the dataset. Those network properties capable of distinguishing learning from memorizing, e.g., Lipschitz constant or margin, must therefore arise as secondary characteristics. They are functions of the dataset the network is trained on.

We want clean descriptions of DNN functions that generalize. By the above discussion, these are the DNNs that inherit some regularizing property from the training data through the gradient descent process. What sort of architecture agnostic language allows for succinct descriptions of trained DNNs exactly when we make some strong assumption about the training set?

% To study this question, we design $3$ different network architectures, {\Archi}, {\Archii}, and {\Archiii}, and $3$ datasets {\Datai}, {\Dataii}, and {\Dataiii}, of increasing "complexity" (both pictured in Appendix Figure \ref{fig:arch_diagrams}) \ref{fig:data_diagrams}). To justify that {\Datai}, {\Dataii}, and {\Dataiii} are of "increasing complexity", we simply note that these datasets are nested by construction, and, as a result, so too are the sets of classifiers that fit the data.


\begin{figure*}
\renewcommand{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.15}
\def\nsbwid{0.15\textwidth}
\def\nsbht{1.4cm}
  \centering
    \begin{tabular}[t]{ccc}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[height=4.2cm,keepaspectratio]{figures/Fig1a.png}
    \caption{Regularizing  Effect of Linearly Separable Data}
    \label{fig:1-a}
\end{subfigure}
    &
        \begin{tabular}{c}% if you add [t], than sub images are pushed down
    %%D1A1%%
         \begin{subfigure}[b]{\nsbwid}
                \centering
                \includegraphics[height=4.2cm,keepaspectratio]{figures/NewFigs/1b.png}
                % \label{fig2:D1A1}

                \caption{{\Datai}}
                \label{fig:1-b}
                % \label{fig2:D1A3}
         \end{subfigure}
        \end{tabular}
&
        \begin{tabular}{c}% if you add [t], than sub images are pushed down
    %%D1A1%%
           \begin{subfigure}[b]{\nsbwid}
                \centering
                \includegraphics[height=4.2cm,keepaspectratio]{figures/NewFigs/1c.png}
                % \label{fig2:D1A1}

                \caption{{\Dataii}}
                \label{fig:1-c}
                % \label{fig2:D1A3}
         \end{subfigure}
        \end{tabular}\\
    \end{tabular}
  \caption{Structural organization of the decision boundary(DB) and NSBs (where each neuron changes from "on" to "off") of trained DNNs as the data (Fig. \ref{fig:1-a}) and architecture complexity varies (Figs.\ref{fig:1-b}, \ref{fig:1-c}). In Fig. \ref{fig:1-a}, \textit{if and only if} we include additional noisy training data to the linearly classifiable {\Datai} can we avoid learning an (essentially) linear classifier. Regularity is not tied to data fit but data structure: all $4$ {\Archiii} classifiers have $0$ training error and vanishing loss on the same original data.
%  However, only the simplest, nearly linear, classifier optically resembles classifiers achievable through gradient descent ("x"s). We hypothesize that gradient descent yields a classifier corresponding to a class with not too much more capacity than is needed to fit the data.
  %
  In columns (\ref{fig:1-b},\ref{fig:1-c}) we plot all NSBs(different linestyle[color] distinguishes NSBs of neurons in different[the same] hidden layer) and the DB(dotted). We see that for fixed dataset, increasing the architecture size (moving down a column) does not qualitatively change the learned DB. Additional layers may add more NSBs, but these organize during training in redundant, parallel shells that do not make the DB more complex. 
%   Describing the decision boundary is sufficient to capture the essential structural motif. 
  Only those NSBs that intersect the DB influence the DB and cause it to bend. Not only is the number of intersections between the DB and NSBs minimized, but also they separate from one another during training, as if by some (regularizing) "repulsive force", most readily apparent in row $2$ col \ref{fig:1-b} (and in the Supplemental animations), that repels the NSBs from the decision boundary. There are several sources of relevant additional information for this figure. The Appendix contains Figures \ref{fig:arch_diagrams} and \ref{fig:data_diagrams}, which are useful to quickly visually appreciate the architectures, ArchI,II,III, and training data, DataI,II,III. It also contains Figure \ref{fig:neuron_states}, which elaborate on these NSB diagrams in number, kind, and size.
  \ref{fig:arch_diagrams} and \ref{fig:data_diagrams}
    }
  \label{fig:unused_capacity}
\end{figure*}
%Noise1,2,3,Actual:
%Loss: 7e-7,2e-3,7e-8,1e-29 But Actual was around 1e-8 for a long time.

%\footnote{It is known that DNNs are robust to label randomization of a subset of the training data. This is potentially a high dimensional phenomenon that is difficult to gain intuition for in 2 dimensions}
\subsection{A Deep Think on Simple Observations}
\begin{displayquote}
\centering
We find in our experiments that DNNs of any architecture trained on linearly classifiable data are almost always linear classifiers (Fig \ref{fig:unused_capacity}).
\end{displayquote}

% \begin{figure}
%   \centering
%   %\includegraphics[width=0.8\linewidth]{arch_diagrams_arabic.pdf}
%   \includegraphics[width=0.8\linewidth]{figures/Fig1a.png}
%   \caption{A scatter plot of {\Datai} and the classification boundaries of $4$ {\Archiii} networks with weights set to various values. All $4$ of these networks have perfect classification accuracy and vanishingly small cross-entropy loss on the data. However, only the simplest, nearly linear, classifier optically resembles classifiers achievable through gradient descent ("x"s).
%   We hypothesize that gradient descent yields a classifier corresponding to a class with not too much more capacity than is needed to fit the data.
%   In fact, the way we generated the $3$ more complicated classifiers was by adding random noise to the dataset before running gradient descent.
% %   However, only the rightmost, center classifier was obtained by training {\Archiii} on {\Datai}, as indicated by the solid, uninterrupted arrow. 
% %   Most often, this classifier will be linear, but we have shown a "typical exception" instead, which is an $AND$ combination of $2$ linear classifiers. 
% % The variety and intricacy of these decision boundaries are reminders of the enormous capacity of {\Archiii}, which has depth $9$ and more than $7e5$ parameters. This capacity is not expressed or apparent in the learned classifier. 
% %   By comparison, the trained classifier appears relatively simple, and has a boundary that consists of two nearly-parallel linear pieces. 
% %   We see that gradient descent is a parsimonious learner that does not merely minimize the training loss and error: it produces complicated decision boundaries if and only if it is required by the data.
%     }
%   \label{fig:unused_capacity}
% \end{figure}




% The reader should keep this example in mind for the entire section.

Is this interesting? Let us consider: though our network has enormous capacity, in this fixed setting of linearly separable data, the deep network behaves as though it has no more capacity than a linear model. When we discuss capacity of a class a functions, we ordinarily consider a hypothesis class consisting of networks indexed over all possible values of weights (or perhaps in a unit ball), since no such restrictions are explicitly built into in the learning algorithm. For a large architecture, such as {\Archiii}, this hypothesis class consists of a tremendous diversity of decision boundaries that fit the data. However, here we observe only a subset of learners: Not every configuration of weights nor every hypothesis is reachable by training with gradient descent on linearly classifiable data. Consider a learning the DNN weights corresponding to the $9$ layer network, {\Archiii}. The VCDim of such hypotheses indexed by every possible weight assignment is $1e6$, which is unhelpfully large. But, have we measured the capacity of the correct class? If we instead use the class reachable by gradient descent, then data assumptions, which are in some form necessary, by constraining the inputs to our learning algorithm in turn restrict our hypothesis class. Linear separability is a particularly strong data assumption which reduces our the VC dimension of our hypothesis class from $1e6$ to $3$. We conclude:
%We conclude by connecting these observations on learning to necessary properties of corresponding learning bounds.

To ensure generalization of unregularized DNN learners, not only are data assumptions \textit{necessary}, but also strong enough assumptions on the training data are themselves \textit{sufficient} for generalization.

% Linearly separable data  in advance that the data is linearly separable is not the norm, but it happens often enough simply out of domain considerations that we might   that the data are linearly separable might simply be implied by the domain of the problem. While knowing the data are linearly separable  mundane-seeming data assumption    we should consider linear separability as an extremely 

% In fact, Conditioned  such data assumptio provide an example where strong assumptions  that   provide an  demonstrate   
% A practitioner with very strong advanced knowledge that the data is linearly separable also may conclude that the DNN returned from training belongs to a class of VC dimension $3$. This , the generalization bound is governed by $3$ instead of $1e6$ , resolving a special case of the paradox.

% A second interesting observation is that linearly separable training data implies the trained network will be \textit{interpretable}, independently of the network architecture. In the next section, we will explore other architecture independent properties related to interpretability.

% The idea of using strictly combinatorial methods, such as VC dimension, appeals to us. Although generalization bounds can always be improved by incorporating additional information like margin and scale, we also want to provide explanations that are as simple as possible. 

% Ultimately though, we are not interested in the special case of linearly separable data, but in what that special case can teach us. To explore whether this paradigm represents a plausible hypothesis for explaining the mismatch between our practical and theoretical expectations for deep learning performance, we need to ask, "do the real-world situations we expect a very deep network to generalize coincide with situations where we have \textit{a priori} knowledge about the dataset?". Yes. In fact, there is a close correspondence between these two. 
% When the practitioner knows in advance that a dataset corresponds to some real-world, human-learnable task, perhaps even one similar to others successfully learned by previous DNN models (e.g. image processing), then the practitioner feels intuitively that a DNN should be able to generalize much better than chance with not too many samples. 
% Conversely, if we the authors in secrecy cook up a data distribution and training set for the reader to train a network on, the reader will not necessarily feel confident that the training and test error should be related.

% \begin{displayquote}
% \centering
%  The properties of trained DNNs which are data dependent but architecture agnostic lie at the \textit{decision boundary}.
% \end{displayquote}

% In Figure \ref{fig:neuron_states}, 
In Figures \ref{fig:1-b},\ref{fig:1-c}, 
we see that a DNN with more parameters learns a more complicated \textit{function} but not a more complicated \textit{classifier}. For example, the number of linear regions does seem to scale with depth for fixed dataset. However, instead of intersecting the decision boundary or one another, these additional NSBs form redundant onion-like structures parallel to the decision boundary.

Since we have argued that learning guarantees in this setting are essentially equivalent to training data guarantees, capacity measures on the learned network $\net$ that imply generalization must somehow reflect the regularity of the data that was originally trained on. Conversely, the factors not determined by the training data structure should \textit{not} factor into the capacity measure. For example, we desire bounds which do not grow with depth.

A capacity measure on $\net(x)$ that is determined entirely by restricting $\net$ to a neighborhood of its decision boundary accomplishes both such goals. The effect of the data is captured because the geometry of this boundary closely mirrors the that of the training data in arrangement and complexity. Consider also that behavior of $\net$ at the decision boundary is still is sufficient to determine each input classification and therefore the generalization analysis is unchanged. We claim  restricting $\net$ to near the decision boundary destroys the architecture information used to parameterize $\net$. More specifically, only the existence of neurons whose NSB intersects the decision boundary can be inferred from observation of inputs $x$ and outputs $\net(x)$ near the boundary. For example, this restriction is the same both for a linear classifier and for a deep network that learns a linear classifier with $50$ linear regions (as in Fig. \ref{fig:1-b}).

% We observe that the complexity and geometry \textit{at the decision boundary} is a key invariant that is sensitive to dataset complexity, inert to architecture changes, and representative of the overall organization of all NSBs. These properties make it a promising candidate for both generalization and interpretability. We build a theory that exploits this observation.

%How this makes sense given gradient descent.

%Invite reader to visit GitHub repo link. TODO
%subsets of neurons whose lines do not intersect share information: not all combo possible.
% Perhaps an aside about K-independence and general position.
% Talk about how number pieces at boundary better invariant than number of pieces

